Calibration Meets Explanation: A Simple and Effective Approach for Model Confidence Estimates

Calibration strengthens the trustworthiness of black-box models by producing better accurate confidence estimates on given examples. However, little is known about if model explanations can help confidence calibration. Intuitively, humans look at important features attributions and decide whether the model is trustworthy. Similarly, the explanations can tell us when the model may or may not know. Inspired by this, we propose a method named CME that leverages model explanations to make the model less confident with non-inductive attributions. The idea is that when the model is not highly confident, it is difficult to identify strong indications of any class, and the tokens accordingly do not have high attribution scores for any class and vice versa. We conduct extensive experiments on six datasets with two popular pre-trained language models in the in-domain and out-of-domain settings. The results show that CME improves calibration performance in all settings. The expected calibration errors are further reduced when combined with temperature scaling. Our findings highlight that model explanations can help calibrate posterior estimates.

==> related.tex <==
\section{Related Work}

Our work is primarily motivated by previous analyses of posterior calibration on modern neural networks. Guo et al. (2017) pointed out that in some cases, as the classification performance of neural networks improves, its posterior output becomes poorly calibrated. There are a few attempts to investigate the effect of posterior calibration on natural language processing (NLP) tasks: Nguyen and O’Connor (2015) empirically tested how classifiers on NLP tasks (e.g., sequence tagging) are calibrated. For instance, compared to the Naive Bayes classifier, logistic regression outputs wellcalibrated posteriors in sentiment classification task. Card and Smith (2018) also mentioned the importance of calibration when generating a training corpus for NLP tasks.

As noted above, numerous post-processing calibration techniques have been developed: traditional binning methods (Zadrozny and Elkan, 2001, 2002) set up bins based on the predicted posterior ˆ p, recalculate calibrated posteriors ˆ q per each bin on a validation set, and then update every ˆ p with ˆ q if ˆ p falls into the certain bin. On the other hand, scaling methods (Platt et al., 1999; Guo et al., 2017; Kull et al., 2019) re-scale the predicted posterior ˆ p from the softmax layer trained on a validation set. Recently, Kumar et al. (2019) pointed out that such re-scaling methods do not actually produce well-calibrated probabilities as reported since the true posterior probability distribution can not be captured with the often low number of samples in the validation set2 . To address the issue, the authors proposed a scaling-binning calibrator, but still rely on the validation set.
